The Initial Properties of Young Star Clusters in M83

The initial sizes and masses of massive star clusters provide information about the cluster formation process and also determine how cluster populations are modified and destroyed, which have implications for using clusters as tracers of galaxy assembly. Young massive cluster populations are often assumed to be unchanged since cluster formation, and therefore their distribution of masses and radii are used as the initial values. However, the first few hundred million years of cluster evolution does change both cluster mass and cluster radius, through both internal and external processes. In this paper, we use a large suite of $N$-body cluster simulations in an appropriate tidal field to determine the best initial mass and initial size distributions of young clusters in the nearby galaxy M83. We find that the initial masses follow a power-law distribution with a slope of -2.7 $\pm$ 0.4, and the half-mass radii follow a log-normal distribution with a mean of 2.57 $\pm$ 0.04 pc and a dispersion of 1.59 $\pm$ 0.01 pc. The corresponding initial projected half-light radius function has a mean of 2.7 $\pm$ 0.3 pc and a dispersion of 1.7 $\pm$ 0.2 pc. The evolution of the initial mass and size distribution functions are consistent with mass loss and expansion due to stellar evolution, independent of the external tidal field and the cluster's initial density profile. Observed cluster sizes and masses should not be used as the initial values, even when clusters are only a few hundred million years old.

==> notes.tex <==
%% Define notes using todonotes package

\usepackage{xparse}
\usepackage{ifthen}

\makeatletter
% Increase margins for margin comments
\ifthenelse{\@todonotes@enable=1 \AND \@todonotes@inline=0}{
\paperwidth=\dimexpr\paperwidth + 6cm\relax
%\textwidth=\dimexpr \textwidth - 6cm\relax
\oddsidemargin=\dimexpr\oddsidemargin + 3cm\relax
\evensidemargin=\dimexpr\evensidemargin + 3cm\relax
\marginparwidth=\dimexpr \marginparwidth + 2.5cm\relax}{}

\ifthenelse{\@todonotes@enable=1}
  {\usepackage[textwidth=\dimexpr\evensidemargin + 2.25cm]{todonotes}}
  {\usepackage[disable]{todonotes}}

% Colors for comment boxes
\definecolor{gold}{RGB}{255,215,0}
\definecolor{salmon}{rgb}{0.95,0.5,0.25}
\definecolor{darkgreen}{rgb}{0.0, 0.5, 0.0}
\definecolor{darkblue}{rgb}{0.0, 0., 0.7}
\definecolor{vlightblue}{rgb}{0.68,0.84,0.9}
\definecolor{purple}{rgb}{0.7, 0., 0.7}
\definecolor{lavender}{rgb}{0.9, 0.9, 0.98}

\newcommand{\@todonotes@loaded}{0}
\@ifpackageloaded{todonotes}
  {\renewcommand{\@todonotes@loaded}{1}}
  {\renewcommand{\@todonotes@loaded}{0}}
% Deal with inline: hack
\ifthenelse{\@todonotes@inline=0}
  {\renewcommand{\@todonotes@loaded}{1}}
  {\renewcommand{\@todonotes@loaded}{0}}
\@ifpackagewith{todonotes}{disable}
  {\renewcommand{\@todonotes@loaded}{0}}
  {}

% Increase margins for margin comments
%\ifthenelse{\@todonotes@loaded=1}{
%\textwidth=\dimexpr \textwidth - 6cm\relax
%\oddsidemargin=\dimexpr\oddsidemargin + 3cm\relax
%\evensidemargin=\dimexpr\evensidemargin + 3cm\relax
%\marginparwidth=\dimexpr \marginparwidth + 2.5cm\relax}{}

\ifthenelse{\@todonotes@inline=1}{
\NewDocumentCommand{\note}{O{black} O{gold} m}{\todo[inline,backgroundcolor={#2},linecolor={#2},bordercolor={#1}]{{\protect\footnotesize #3}}}}
{\NewDocumentCommand{\note}{O{black} O{gold} m}{\todo[backgroundcolor={#2},linecolor={#2},bordercolor={#1}]{{\protect\footnotesize #3}}}}
\makeatother
